Parity-Violating Observables of Two-Nucleon Systems in Effective Field Theory

A newly-proposed parity-violating nucleon-nucleon interaction based on effective field theory is studied in this work. It is found that at low energy, i.e., E_lab less than 90 MeV for 1S0-3P0 transitions and E_lab less than 40 MeV for 3S1-1P1 and 3S1-3P1 transitions, the parity-violating observables can be completely specified by a minimal set of six parameters. It contains five low-energy constants, which are equivalent to the Danilov parameters, and an additional parameter that characterizes the long-range one-pion exchange and is proportional to the parity-violating pion-nucleon coupling constant. Selected observables in two-nucleons systems are analyzed in this framework with their dependence on these parameters being expressed in a nearly model-independent way.

==> tmp/my_macro.tex <==
\usepackage{bm}
\usepackage{slashed}
\usepackage{braket}
\usepackage{nicefrac}

%\newcommand{\etal}{\textit{et al.}}

\newcommand{\dst}[1]{\displaystyle{#1}}
\newcommand{\tst}[1]{\textstyle{#1}}
\newcommand{\mtst}[1]{{\tiny #1}}
\newcommand{\sst}[1]{\scriptstyle{#1}}
\newcommand{\ssst}[1]{\scriptscriptstyle{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}

%\newcommand{\bra}[1]{\langle #1 \vert}
%\newcommand{\ket}[1]{\vert #1 \rangle}
%\newcommand{\expec}[1]{\langle #1 \rangle}

\newcommand{\mN}{m_{\ssst{N}}}
\newcommand{\sstw}{\sin^2\theta_W}

\newcommand{\GMs}{G_{\ssst{M}}^{(s)}}
\newcommand{\GAeV}{G_{\ssst{A}}^{(e)\,\sst{(T=1)}}}
\newcommand{\gAe}{g_{\ssst{A}}^{e}}
\newcommand{\gVe}{g_{\ssst{V}}^{e}}


\newcommand{\WEM}{W^{\ssst{EM}}}
\newcommand{\WPV}{W^{\ssst{PV}}}
\newcommand{\WPVZ}{W^{\ssst{PV(Z)}}}
\newcommand{\WPVg}{W^{\ssst{PV}(\gamma)}}
\newcommand{\ALR}{A_{\ssst{LR}}}
\newcommand{\ALRZ}{A_{\ssst{LR}}^{(Z)}}
\newcommand{\ALRg}{A_{\ssst{LR}}^{(\gamma)}}

\newcommand{\vect}{\vec{\tau}}
\newcommand{\vecs}{\vec{\sigma}}

\newcommand{\gpiNN}{g_{\pi\ssst{NN}}}
\newcommand{\getaNN}{g_{\eta\ssst{NN}}}
\newcommand{\grhoNN}{g_{\rho\ssst{NN}}}
\newcommand{\gomegaNN}{g_{\omega\ssst{NN}}}

\newcommand{\muS}{\mu_{\ssst{S}}}
\newcommand{\muV}{\mu_{\ssst{V}}}
\newcommand{\chiS}{\chi_{\ssst{S}}}
\newcommand{\chiV}{\chi_{\ssst{V}}}
\newcommand{\kappaS}{\kappa_{\ssst{S}}}
\newcommand{\kappaV}{\kappa_{\ssst{V}}}

\newcommand{\PV}{\slashed{P}}
\newcommand{\HPV}{H_{\ssst{\slashed{P}}}}
\newcommand{\TV}{\slashed{T}}
\newcommand{\PVTV}{\slashed{P}\slashed{T}}
\newcommand{\HPVTV}{H_{\ssst{\slashed{P}\slashed{T}}}}

